Quantum Computing through Computational Imaging: Representations, Measurement, and Inference

An algebraic correspondence between an imaging model and a quantum state does not specify a computational method: input access, measurement and decoding determine what can be returned. This exposition develops four distinctions for computational-imaging and engineering readers. It separates amplitude encodings of input values from encodings of complete candidate labelings, explaining why amplitude storage does not provide full-array readout. Complex-field interference motivates unknown-phase inference: complementary measurements resolve ambiguities that local Fisher information alone does not detect. Reshaping joint amplitudes into a matrix connects singular-value decomposition to pure-state entanglement, while distinguishing Schmidt rank from conditions for efficient classical simulation. In a four-pixel segmentation, an objective becomes a cost operator and a sampling circuit. One layer of the quantum approximate optimization algorithm (QAOA) lowers mean energy from $1.675$ to $0.686$ relative to uniform sampling, yet makes a nonoptimal labeling more probable than the optimum 0.484 versus 0.365. Archived IBM and IQM measurements illustrate a separate six-variable local boundary decision. Low-rank state reconstruction and selected quantum algorithms connect these distinctions to an end-to-end resource account. The derivations and reproducible numerical references assume complex linear algebra and probability, without prior quantum mechanics. The accompanying Seeing Amplitudes browser laboratory supports interactive exploration; the article remains self-contained and connects each representation to the estimate or decision it permits and the resources that output requires.

==> figures/figure_style.tex <==
% Vector figures for the compact two-column arXiv article.
% Latin Modern Sans labels use the article's normal mathematical fonts.
\colorlet{FigureTeal}{accent}
\colorlet{FigureSoft}{boxbg}
\definecolor{FigureInk}{HTML}{173348}
\definecolor{FigureOchre}{HTML}{B26F19}
\definecolor{FigureMuted}{HTML}{465963}
\newcommand{\figfamily}{\fontencoding{T1}\fontfamily{lmss}\fontshape{n}}
% Fixed readable label sizes; wide drawings shrink only when they exceed the line.
\newcommand{\figtext}{\figfamily\fontseries{m}\fontsize{9}{10.8}\selectfont\mathversion{normal}}
\newcommand{\figsmall}{\figfamily\fontseries{m}\fontsize{8}{9.6}\selectfont\mathversion{normal}}
\newcommand{\figtitle}{\figfamily\fontseries{bx}\fontsize{9}{10.8}\selectfont\mathversion{normal}}

\tikzset{
 % Base for every picture in a figure float (applied below).
 exposition figure/.style={execute at begin picture={\figtext},text=FigureInk,
  line join=round,line cap=round,>={Stealth[length=2mm,width=1.5mm]}},
 fig box/.style={draw=FigureInk!55,fill=FigureSoft,rounded corners=1.5pt,
  line width=.5pt,align=center,inner sep=3pt,text=FigureInk},
 fig plain box/.style={fig box,fill=white},
 fig arrow/.style={-{Stealth[length=2mm,width=1.5mm]},line width=.55pt,draw=FigureInk},
 fig guide/.style={line width=.4pt,draw=FigureMuted!60},
 % Quantum circuits: single quantum wires, double classical wires after measurement.
 qwire/.style={line width=.55pt,draw=FigureInk},
 cwire/.style={double=white,double distance=1pt,line width=.4pt,draw=FigureInk},
 gate/.style={draw=FigureTeal,line width=.55pt,fill=FigureSoft,minimum height=5.2mm,
  minimum width=6mm,inner sep=1.8pt,text=FigureInk},
 meter/.pic={\draw[line width=.55pt,draw=FigureInk,fill=white] (-3mm,-2.6mm) rectangle (3mm,2.6mm);
  \draw[line width=.45pt,draw=FigureInk] (-1.95mm,-1.1mm) arc (180:0:1.95mm);
  \draw[line width=.45pt,draw=FigureInk,-{Stealth[length=1mm,width=.85mm]}] (0,-1.1mm)--(1.4mm,1.7mm);},
 ctrl/.style={circle,fill=FigureInk,inner sep=0pt,minimum size=1.6mm},
 targ/.pic={\draw[line width=.55pt,draw=FigureInk,fill=white] (0,0) circle (1.6mm);
  \draw[line width=.55pt,draw=FigureInk] (-1.6mm,0)--(1.6mm,0) (0,-1.6mm)--(0,1.6mm);},
}
\AtBeginEnvironment{figure}{\tikzset{every picture/.append style={exposition figure}}}
\AtBeginEnvironment{figure*}{\tikzset{every picture/.append style={exposition figure}}}
\pgfplotsset{exposition axis/.style={font=\figtext,label style={font=\figtext},
 tick label style={font=\figsmall},/pgf/number format/assume math mode=true}}
\AtBeginEnvironment{figure}{\pgfplotsset{every axis/.append style={exposition axis}}}
\AtBeginEnvironment{figure*}{\pgfplotsset{every axis/.append style={exposition axis}}}

